CP-violating inflation and its cosmological imprints

We study models with several $SU(2)$ scalar doublets where the inert doublets have a non-minimal coupling to gravity and play the role of the inflaton. We allow for this coupling to be complex, thereby introducing CP-violation -- a necessary source of the baryon asymmetry -- in the Higgs-inflaton couplings. We investigate the inflationary dynamics of the model and discuss how the CP-violation of the model is imprinted on the particle asymmetries after inflation in the hot big bang universe.

==> CPV-inflation_KT_VK-references.tex <==
%\cite{Aad:2012tfa}
\bibitem{Aad:2012tfa}
G.~Aad \textit{et al.} [ATLAS],
%``Observation of a new particle in the search for the Standard Model Higgs boson with the ATLAS detector at the LHC,''
Phys. Lett. B \textbf{716}, 1-29 (2012)
doi:10.1016/j.physletb.2012.08.020
[arXiv:1207.7214 [hep-ex]].
%11946 citations counted in INSPIRE as of 15 Feb 2021

%\cite{Chatrchyan:2012ufa}
\bibitem{Chatrchyan:2012ufa}
S.~Chatrchyan \textit{et al.} [CMS],
%``Observation of a New Boson at a Mass of 125 GeV with the CMS Experiment at the LHC,''
Phys. Lett. B \textbf{716}, 30-61 (2012)
doi:10.1016/j.physletb.2012.08.021
[arXiv:1207.7235 [hep-ex]].
%11651 citations counted in INSPIRE as of 15 Feb 2021

%\cite{Ade:2015xua}
\bibitem{Ade:2015xua}
P.~A.~R.~Ade \textit{et al.} [Planck],
%``Planck 2015 results. XIII. Cosmological parameters,''
Astron. Astrophys. \textbf{594}, A13 (2016)
doi:10.1051/0004-6361/201525830
[arXiv:1502.01589 [astro-ph.CO]].
%9550 citations counted in INSPIRE as of 13 Feb 2021

%\cite{Morrissey:2012db}
\bibitem{Morrissey:2012db}
D.~E.~Morrissey and M.~J.~Ramsey-Musolf,
%``Electroweak baryogenesis,''
New J. Phys. \textbf{14}, 125003 (2012)
doi:10.1088/1367-2630/14/12/125003
[arXiv:1206.2942 [hep-ph]].
%496 citations counted in INSPIRE as of 03 Feb 2021

%\cite{Gavela:1993ts}
\bibitem{Gavela:1993ts}
M.~B.~Gavela, P.~Hernandez, J.~Orloff and O.~Pene,
%``Standard model CP violation and baryon asymmetry,''
Mod. Phys. Lett. A \textbf{9}, 795-810 (1994)
doi:10.1142/S0217732394000629
[arXiv:hep-ph/9312215 [hep-ph]].
%374 citations counted in INSPIRE as of 25 Jan 2021

%\cite{Huet:1994jb}
\bibitem{Huet:1994jb}
P.~Huet and E.~Sather,
%``Electroweak baryogenesis and standard model CP violation,''
Phys. Rev. D \textbf{51}, 379-394 (1995)
doi:10.1103/PhysRevD.51.379
[arXiv:hep-ph/9404302 [hep-ph]].
%450 citations counted in INSPIRE as of 22 Jan 2021

%\cite{Gavela:1994dt}
\bibitem{Gavela:1994dt}
M.~B.~Gavela, P.~Hernandez, J.~Orloff, O.~Pene and C.~Quimbay,
%``Standard model CP violation and baryon asymmetry. Part 2: Finite temperature,''
Nucl. Phys. B \textbf{430}, 382-426 (1994)
doi:10.1016/0550-3213(94)00410-2
[arXiv:hep-ph/9406289 [hep-ph]].
%403 citations counted in INSPIRE as of 22 Jan 2021

%\cite{Kajantie:1995kf}
\bibitem{Kajantie:1995kf}
K.~Kajantie, M.~Laine, K.~Rummukainen and M.~E.~Shaposhnikov,
%``The Electroweak phase transition: A Nonperturbative analysis,''
Nucl. Phys. B \textbf{466}, 189-258 (1996)
doi:10.1016/0550-3213(96)00052-1
[arXiv:hep-lat/9510020 [hep-lat]].
%420 citations counted in INSPIRE as of 22 Jan 2021

%\cite{Hawking:1982cz}
\bibitem{Hawking:1982cz}
S.~W.~Hawking,
%``The Development of Irregularities in a Single Bubble Inflationary Universe,''
Phys. Lett. B \textbf{115}, 295 (1982)
doi:10.1016/0370-2693(82)90373-2
%1874 citations counted in INSPIRE as of 15 Feb 2021

%\cite{Starobinsky:1982ee}
\bibitem{Starobinsky:1982ee}
A.~A.~Starobinsky,
%``Dynamics of Phase Transition in the New Inflationary Universe Scenario and Generation of Perturbations,''
Phys. Lett. B \textbf{117}, 175-178 (1982)
doi:10.1016/0370-2693(82)90541-X
%2349 citations counted in INSPIRE as of 15 Feb 2021

%\cite{Sasaki:1986hm}
\bibitem{Sasaki:1986hm}
M.~Sasaki,
%``Large Scale Quantum Fluctuations in the Inflationary Universe,''
Prog. Theor. Phys. \textbf{76}, 1036 (1986)
doi:10.1143/PTP.76.1036
%509 citations counted in INSPIRE as of 02 Feb 2021

%\cite{Mukhanov:1988jd}
\bibitem{Mukhanov:1988jd}
V.~F.~Mukhanov,
%``Quantum Theory of Gauge Invariant Cosmological Perturbations,''
Sov. Phys. JETP \textbf{67}, 1297-1302 (1988)
%385 citations counted in INSPIRE as of 03 Feb 2021

%\cite{Bezrukov:2007ep}
\bibitem{Bezrukov:2007ep}
F.~L.~Bezrukov and M.~Shaposhnikov,
%``The Standard Model Higgs boson as the inflaton,''
Phys. Lett. B \textbf{659}, 703-706 (2008)
doi:10.1016/j.physletb.2007.11.072
[arXiv:0710.3755 [hep-th]].
%1493 citations counted in INSPIRE as of 10 Feb 2021

%\cite{Lerner:2009xg}
\bibitem{Lerner:2009xg}
R.~N.~Lerner and J.~McDonald,
%``Gauge singlet scalar as inflaton and thermal relic dark matter,''
Phys. Rev. D \textbf{80}, 123507 (2009)
doi:10.1103/PhysRevD.80.123507
[arXiv:0909.0520 [hep-ph]].
%190 citations counted in INSPIRE as of 05 Feb 2021

%\cite{Enqvist:2014zqa}
\bibitem{Enqvist:2014zqa}
K.~Enqvist, S.~Nurmi, T.~Tenkanen and K.~Tuominen,
%``Standard Model with a real singlet scalar and inflation,''
JCAP \textbf{08}, 035 (2014)
doi:10.1088/1475-7516/2014/08/035
[arXiv:1407.0659 [astro-ph.CO]].
%58 citations counted in INSPIRE as of 31 Jan 2021

%\cite{Gong:2012ri}
\bibitem{Gong:2012ri}
J.~O.~Gong, H.~M.~Lee and S.~K.~Kang,
%``Inflation and dark matter in two Higgs doublet models,''
JHEP \textbf{04}, 128 (2012)
doi:10.1007/JHEP04(2012)128
[arXiv:1202.0288 [hep-ph]].
%45 citations counted in INSPIRE as of 22 Jan 2021

%\cite{Choubey:2017hsq}
\bibitem{Choubey:2017hsq}
S.~Choubey and A.~Kumar,
%``Inflation and Dark Matter in the Inert Doublet Model,''
JHEP \textbf{11}, 080 (2017)
doi:10.1007/JHEP11(2017)080
[arXiv:1707.06587 [hep-ph]].
%19 citations counted in INSPIRE as of 12 Feb 2021

%\cite{Englert:2011yb}
\bibitem{Englert:2011yb}
C.~Englert, T.~Plehn, D.~Zerwas and P.~M.~Zerwas,
%``Exploring the Higgs portal,''
Phys. Lett. B \textbf{703}, 298-305 (2011)
doi:10.1016/j.physletb.2011.08.002
[arXiv:1106.3097 [hep-ph]].
%202 citations counted in INSPIRE as of 04 Feb 2021

%\cite{Branco:2011iw}
\bibitem{Branco:2011iw}
G.~C.~Branco, P.~M.~Ferreira, L.~Lavoura, M.~N.~Rebelo, M.~Sher and J.~P.~Silva,
%``Theory and phenomenology of two-Higgs-doublet models,''
Phys. Rept. \textbf{516}, 1-102 (2012)
doi:10.1016/j.physrep.2012.02.002
[arXiv:1106.0034 [hep-ph]].
%1956 citations counted in INSPIRE as of 09 Feb 2021

%\cite{Keus:2016orl}
\bibitem{Keus:2016orl}
V.~Keus,
%``CP violation and BSM Higgs bosons,''
PoS \textbf{CHARGED2016}, 017 (2016)
doi:10.22323/1.286.0017
[arXiv:1612.03629 [hep-ph]].
%4 citations counted in INSPIRE as of 22 Jan 2021

%\cite{Cordero-Cid:2016krd}
\bibitem{Cordero-Cid:2016krd}
A.~Cordero-Cid, J.~Hern\'andez-S\'anchez, V.~Keus, S.~F.~King, S.~Moretti, D.~Rojas and D.~Soko\l{}owska,
%``CP violating scalar Dark Matter,''
JHEP \textbf{12}, 014 (2016)
doi:10.1007/JHEP12(2016)014
[arXiv:1608.01673 [hep-ph]].
%18 citations counted in INSPIRE as of 04 Feb 2021

%\cite{Cordero:2017owj}
\bibitem{Cordero:2017owj}
A.~Cordero, J.~Hernandez-Sanchez, V.~Keus, S.~F.~King, S.~Moretti, D.~Rojas and D.~Sokolowska,
%``Dark Matter Signals at the LHC from a 3HDM,''
JHEP \textbf{05}, 030 (2018)
doi:10.1007/JHEP05(2018)030
[arXiv:1712.09598 [hep-ph]].
%10 citations counted in INSPIRE as of 04 Feb 2021

%\cite{Cordero-Cid:2018man}
\bibitem{Cordero-Cid:2018man}
A.~Cordero-Cid, J.~Hern\'andez-S\'anchez, V.~Keus, S.~Moretti, D.~Rojas and D.~Soko\l{}owska,
%``Lepton collider indirect signatures of dark CP-violation,''
Eur. Phys. J. C \textbf{80}, no.2, 135 (2020)
doi:10.1140/epjc/s10052-020-7689-0
[arXiv:1812.00820 [hep-ph]].
%6 citations counted in INSPIRE as of 04 Feb 2021

%\cite{Cordero-Cid:2020yba}
\bibitem{Cordero-Cid:2020yba}
A.~Cordero-Cid, J.~Hern\'andez-S\'anchez, V.~Keus, S.~Moretti, D.~Rojas-Ciofalo and D.~Soko\l{}owska,
%``Collider signatures of dark $CP$-violation,''
Phys. Rev. D \textbf{101}, no.9, 095023 (2020)
doi:10.1103/PhysRevD.101.095023
[arXiv:2002.04616 [hep-ph]].
%7 citations counted in INSPIRE as of 04 Feb 2021

%\cite{Keus:2020ooy}
\bibitem{Keus:2020ooy}
V.~Keus,
%``Dark origins of matter-antimatter asymmetry,''
PoS \textbf{CORFU2019}, 059 (2020)
doi:10.22323/1.376.0059
[arXiv:2003.02141 [hep-ph]].
%1 citations counted in INSPIRE as of 22 Jan 2021

%\cite{Keus:2019szx}
\bibitem{Keus:2019szx}
V.~Keus,
%``Dark CP-violation through the $Z$-portal,''
Phys. Rev. D \textbf{101}, no.7, 073007 (2020)
doi:10.1103/PhysRevD.101.073007
[arXiv:1909.09234 [hep-ph]].
%5 citations counted in INSPIRE as of 01 Feb 2021

%\cite{Ahriche:2015mea}
\bibitem{Ahriche:2015mea}
A.~Ahriche, G.~Faisel, S.~Y.~Ho, S.~Nasri and J.~Tandean,
%``Effects of two inert scalar doublets on Higgs boson interactions and the electroweak phase transition,''
Phys. Rev. D \textbf{92}, no.3, 035020 (2015)
doi:10.1103/PhysRevD.92.035020
[arXiv:1501.06605 [hep-ph]].
%16 citations counted in INSPIRE as of 04 Feb 2021

%\cite{Ivanov:2011ae}
\bibitem{Ivanov:2011ae}
I.~P.~Ivanov, V.~Keus and E.~Vdovin,
%``Abelian symmetries in multi-Higgs-doublet models,''
J. Phys. A \textbf{45}, 215201 (2012)
doi:10.1088/1751-8113/45/21/215201
[arXiv:1112.1660 [math-ph]].
%63 citations counted in INSPIRE as of 22 Jan 2021

%\cite{Keus:2013hya}
\bibitem{Keus:2013hya}
V.~Keus, S.~F.~King and S.~Moretti,
%``Three-Higgs-doublet models: symmetries, potentials and Higgs boson masses,''
JHEP \textbf{01}, 052 (2014)
doi:10.1007/JHEP01(2014)052
[arXiv:1310.8253 [hep-ph]].
%58 citations counted in INSPIRE as of 22 Jan 2021

%\cite{Kaiser:2010ps}
\bibitem{Kaiser:2010ps}
D.~I.~Kaiser,
%``Conformal Transformations with Multiple Scalar Fields,''
Phys. Rev. D \textbf{81}, 084044 (2010)
doi:10.1103/PhysRevD.81.084044
[arXiv:1003.1159 [gr-qc]].
%117 citations counted in INSPIRE as of 04 Feb 2021

%\cite{Ade:2015lrj}
\bibitem{Ade:2015lrj}
P.~A.~R.~Ade \textit{et al.} [Planck],
%``Planck 2015 results. XX. Constraints on inflation,''
Astron. Astrophys. \textbf{594}, A20 (2016)
doi:10.1051/0004-6361/201525898
[arXiv:1502.02114 [astro-ph.CO]].
%2220 citations counted in INSPIRE as of 08 Feb 2021

%\cite{Komatsu:2010fb}
\bibitem{Komatsu:2010fb}
E.~Komatsu \textit{et al.} [WMAP],
%``Seven-Year Wilkinson Microwave Anisotropy Probe (WMAP) Observations: Cosmological Interpretation,''
Astrophys. J. Suppl. \textbf{192}, 18 (2011)
doi:10.1088/0067-0049/192/2/18
[arXiv:1001.4538 [astro-ph.CO]].
%7085 citations counted in INSPIRE as of 15 Feb 2021

%\cite{Linde:1981mu}
\bibitem{Linde:1981mu}
A.~D.~Linde,
%``A New Inflationary Universe Scenario: A Possible Solution of the Horizon, Flatness, Homogeneity, Isotropy and Primordial Monopole Problems,''
Phys. Lett. B \textbf{108}, 389-393 (1982)
doi:10.1016/0370-2693(82)91219-9
%5162 citations counted in INSPIRE as of 15 Feb 2021
